A p-adaptive polytopal discontinuous Galerkin method for high-order approximation of brain electrophysiology

Multiscale mathematical models have shown great promise in computational brain electrophysiology but are still hindered by high computational costs due to fast dynamics and complex brain geometries, requiring very fine spatio-temporal resolution. This paper introduces a novel p-adaptive discontinuous Galerkin method on polytopal grids (PolyDG) coupled with Crank-Nicolson time integration to approximate such models efficiently. The p-adaptive method enhances local accuracy via dynamic, element-wise polynomial refinement/de-refinement guided by a-posteriori error estimators. A novel clustering algorithm automatizes the selection of elements for adaptive updates, further improving efficiency. A wide set of numerical tests, including epileptic seizure simulations in a sagittal section of a human brain stem, demonstrate the method's ability to reduce computational load while maintaining the accuracy of the numerical solution in capturing the dynamics of multiple wavefronts.

==> comparison_indicator.tex <==
\begin{comment}
\begin{figure}[h!]
\vspace{-0.2cm}
  \centering
\hspace{-3ex}\begin{tabular}{@{}m{2cm} m{9.8cm}@{}} % colonna testo + colonna immagini
    % --- Riga 1 ---
     & 
\hspace{8em}\includegraphics[scale=0.14]{singlewave_stationary/scale_.png}
    \\[-0.1cm]
    \footnotesize{Numerical solution} &
    \includegraphics[trim={2cm 13cm 2cm 13cm},clip, scale=0.065]{comparisontau/sol.png}
    \includegraphics[trim={2cm 13cm 2cm 13cm},clip, scale=0.065]{comparisontau/sol.png}
    \\[-0.8cm]
    % --- Riga 2 ---
 &
\hspace{2em}\includegraphics[trim={2cm 8cm 2cm 8cm},clip, scale=0.16]{singlewave_stationary/scale_p.png}\hspace{5em}\includegraphics[trim={2cm 8cm 2cm 8cm},clip, scale=0.16]{comparisontau/tot_scale.png} 
    \\[0.85cm]
    % --- Riga 3 ---
     \footnotesize{Complete indicator ($\tau_K$)} &
   \includegraphics[trim={2cm 8cm 2cm 8cm},clip, scale=0.065]{comparisontau/total_p.png}\includegraphics[trim={2cm 8cm 2cm 8cm},clip, scale=0.065]{comparisontau/total_t.png} 
\\[-1.2cm]
% --- Riga 3 ---
&\hspace{16em}\includegraphics[trim={2cm 8cm 2cm 8cm},clip, scale=0.16]{comparisontau/jump_scale.png} 
    \\[0.85cm]
% --- Riga 3 ---
    \footnotesize{Jump indicator ($\tau_{K,j}$)} &
    \includegraphics[trim={2cm 8cm 2cm 8cm},clip, scale=0.065]{comparisontau/jump_p.png}  \includegraphics[trim={2cm 8cm 2cm 8cm},clip, scale=0.065]{comparisontau/jump_t.png}
\\[-1.15cm]
&\hspace{16em}\includegraphics[trim={2cm 8cm 2cm 8cm},clip, scale=0.16]{comparisontau/res_scale.png} 
    \\[0.85cm]
    % --- Riga 3 ---
    \footnotesize{Residual indicator ($\tau_{K,r}$)} &
    \includegraphics[trim={2cm 8cm 2cm 8cm},clip, scale=0.065]{comparisontau/residual_p.png}  \includegraphics[trim={2cm 8cm 2cm 8cm},clip, scale=0.065]{comparisontau/residual_t.png}
  \end{tabular}
  \caption{Test case of Subsection~\ref{sec::comparison}. Different local error indicators employed to drive the $p$-adaptive algorithm. The polynomial degree distribution and the computed element-wise indicators at time
$t = 2ms$ are reported.}  \label{fig::comparison_tau}
\end{figure}
\end{comment}

\begin{figure}[h!]
\centering
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.0}
\begin{tabular}{c c c c}
% --- Barre condivise (L2, p, DG) ---
 & 
\multicolumn{3}{c}{%
  \hspace{-4ex}\includegraphics[trim={0 0cm 0 0cm},clip, scale=0.16]{singlewave_stationary/scale_.png}} \\
% --- Riga (i) ---
\raisebox{7mm}{(i)} &
\includegraphics[trim={2cm 13cm 2cm 13cm},clip, scale=0.065]{comparisontau/sol.png} &
\includegraphics[trim={2cm 13cm 2cm 13cm},clip, scale=0.065]{comparisontau/sol.png} &
\includegraphics[trim={2cm 13cm 2cm 13cm},clip, scale=0.065]{comparisontau/sol.png} \\
% --- Riga (ii) ---
 & 
\multicolumn{3}{c}{%
  \includegraphics[trim={0 0cm 0 0cm},clip, scale=0.16]{singlewave_stationary/scale_p.png}} \\
\raisebox{7mm}{(ii)} &
\includegraphics[trim={2cm 13cm 2cm 13cm},clip, scale=0.065]{comparisontau/total_p.png} &
\includegraphics[trim={2cm 13cm 2cm 13cm},clip, scale=0.065]{comparisontau/jump_p.png} &
\includegraphics[trim={2cm 13cm 2cm 13cm},clip, scale=0.065]{comparisontau/residual_p.png} \\
&
\multicolumn{3}{c}{
  \includegraphics[trim={0 0cm 0 0cm},clip, scale=0.16]{newcomp/L2scale.png}
}\\
% --- Riga (iii) ---
\raisebox{7mm}{(iii)} &
\includegraphics[trim={2cm 13cm 2cm 13cm},clip, scale=0.065]{newcomp/L2complete.png} &
\includegraphics[trim={2cm 13cm 2cm 13cm},clip, scale=0.065]{newcomp/jumpL2.png} &
\includegraphics[trim={2cm 13cm 2cm 13cm},clip, scale=0.065]{newcomp/ResidualL2_.png} \\
&
\multicolumn{3}{c}{
     \includegraphics[trim={0 0cm 0 0cm},clip, scale=0.18]{newcomp/DGscale.png}
} \\
% --- Riga (iv) ---
\raisebox{7mm}{(iv)} &
\includegraphics[trim={2cm 13cm 2cm 13cm},clip, scale=0.065]{newcomp/completeDG.png} &
\includegraphics[trim={2cm 13cm 2cm 13cm},clip, scale=0.065]{newcomp/JumpDG.png} &
\includegraphics[trim={2cm 13cm 2cm 13cm},clip, scale=0.065]{newcomp/ResidualDG_.png} \\
& \includegraphics[trim={0 0cm 0 0cm},clip, scale=0.16]{comparisontau/tot_scale.png}
 &  \includegraphics[trim={0 0cm 0 0cm},clip, scale=0.16]{comparisontau/jump_scale.png}  &   \includegraphics[trim={0 0cm 0 0cm},clip, scale=0.16]{comparisontau/res_scale.png} \\
% --- Riga (v) ---
\raisebox{7mm}{(v)} &
  \includegraphics[trim={2cm 13cm 2cm 13cm},clip, scale=0.065]{comparisontau/total_t.png}
&
  \includegraphics[trim={2cm 13cm 2cm 13cm},clip, scale=0.065]{comparisontau/jump_t.png}
&

  \includegraphics[trim={2cm 13cm 2cm 13cm},clip, scale=0.065]{comparisontau/residual_t.png}\\
% --- Caption indicatori ---
 & (a) $\tau_K$ & (b) $\tau_{K,j}$ & (c) $\tau_{K,r}$
\end{tabular}

\caption{Test case of Subsection~\ref{sec::comparison}. Different local error indicators are employed to drive the $p$-adaptive algorithm. The polynomial degree distribution and the computed element-wise indicators at time
$t = 2ms$ are reported. (i) numerical solution: (ii) polynomial degree distribution; (iii) $L2-$norm error distribution; (iv) $DG$-norm error distribution; (v) Indicator distribution.}
\label{fig::comparison_tau}
\end{figure}



==> heterog.tex <==
\vspace{-0.1cm}
\subsubsection{Heterogeneous case} \label{sec:HeteroCase}
In this test case, we instead consider a heterogeneous conductivity tensor that makes the two waves travel at different speeds and with different slopes. This test was designed to assess the ability of the adaptive algorithm to capture two distinct waves with different dynamics. 
For this simulation, we consider a discontinuous conductivity tensor. 
$$
\Sigma(\mathbf{x}) = \Sigma_1 \mathbb{I}_{\Omega_1}(\mathbf{x}) + \Sigma_2 \mathbb{I}_{\Omega_2}(\mathbf{x}), 
$$
changing between the subdomains $\Omega_1 = (-2,1) \times (-0.5,0.5)$ and $\Omega_2 = (1,4) \times (-0.5,0.5)$ (see, e.g., Figure \ref{fig:double_initial_hetero}).  $\Sigma_1$ and $\Sigma_2$ are defined by exploiting the formula for the exact wave velocity in \cite{pezzuto2016space}:  
imposing the wave speed as $c_1 = 0.5 \text{ mm} \cdot \cdot \text{ms}^{-1}$ and $c_2 = 1 \cdot \text{ mm} \cdot \text{ms}^{-1}$ we obtain the conductivity values defined as:
\begin{equation}
    \begin{aligned}
      \Sigma_1 = \begin{bmatrix}
          0.0081 & 0 \\ 0 & 0.0081
      \end{bmatrix} \; , \; \Sigma_2 = \begin{bmatrix}
          0.0551 & 0 \\ 0 & 0.0551
      \end{bmatrix}.
\end{aligned}
\label{eq:sigma_doublewave}
\end{equation}
This choice results in a faster wave evolving from the right to the left of the domain until it encounters a jump in conductivity at $\hat{x}=1$; after that, the wave slows down and becomes steep exactly like the other one, evolving with the same speed.
\begin{figure}[h!]
\centering
\begin{minipage}[b]{0.45\textwidth}
\centering
\includegraphics[trim={2cm 13cm 2cm 13cm},clip,scale=0.075]{doubleheterostationary/setup.png}
\vspace{-10ex}
\begin{center}
\Large $\Omega_1$ \hspace{4em}  $\Omega_2$
\end{center}
\vspace{2ex}
\label{fig:hetero_mesh}
\vspace{-2ex}
%\hspace{0.05\textwidth} % Spazio tra le due figure
\includegraphics[trim={0cm 0cm 0cm 0cm},clip,scale=0.19]{singlewave_stationary/scale_.png}
\hspace{-0.6em}\includegraphics[trim={2cm 13cm 2cm 13cm},clip, scale=0.075]{doubleheterostationary/initial_.png}
\vspace{-0.1cm}
\subcaption{\label{fig:double_initial_hetero}}
\end{minipage}\hfill
\begin{minipage}[b]{0.45\textwidth}
\centering
\begin{tikzpicture}[scale=.5, transform shape]
\begin{axis}[
    width=4.6in,
    height=2.8in,
    domain=-3:5,
    samples=1000,
    xmin=-2, xmax=5,
    ymin=-89, ymax=34,
    xlabel={\footnotesize $x$},
    ylabel={\footnotesize $y$},
    ytick={-85, -60, -40, -20, 0, 10, 30},
    grid=both,
    minor tick num=1,
    axis lines=middle,
    enlargelimits=true,
    tick style={black},
    xmajorgrids, ymajorgrids,
    tick label style={font=\small},
]
\addplot[blue, thick, line width = 1.4pt] {115/2 * (tanh((x - 2.5)/0.4) - tanh((x + 1.5)/0.1)) + 30};
\end{axis}
\end{tikzpicture}
\vspace{0.1cm}
\subcaption{\label{fig:profile}}
\end{minipage}
\caption{Test case of Section~\ref{sec:HeteroCase}. (\ref{fig:double_initial_hetero}) Initial condition for double traveling wavefront ($x_1 = -1.5$, $x_2 = 3$); (\ref{fig:profile}) Profile of the initial condition with the double wave in the heterogeneous domain ($x_1 = -1.5$, $x_2 = 2.5$).}
\end{figure}
The profile of the initial condition is shown in Figure \ref{fig:profile}. 
The distribution of the local polynomial degree differs for the faster wave with a less steep slope (starting in $x_2 = 2.5$). There is a wider band with a different distribution of the local polynomial degree resulting from the fact that the indicator value in correspondence of the second wave is significantly lower. Figure \ref{fig:ndof_evolution_doublehetero} shows the evolution of the NDof and the number of elements for each polynomial degree. With respect to the homogeneous test case analyzed in \ref{sec:HomogCase}, we observe an increase in the total number of degrees of freedom (compare, e.g., Figure \ref{fig:dof_evolution_doubletvh}). The change in wave speed makes the adaptive algorithm increase the high-order polynomial band for the second wave. 
\begin{comment}
\begin{figure}[h!]
\vspace*{-0.4cm}
\begin{subfigure}[b]{0.33\textwidth}
 \hspace*{-1em}\includegraphics[trim={1cm 2cm 0 2cm},clip, scale=0.085]{doubleheterostationary/cluster11.png} \caption{$t = 1.5 \; \mathrm{ms}$}\label{fig::cluster1hetero} 
  \end{subfigure}
    \begin{subfigure}[b]{0.33\textwidth}
 \hspace*{-3em}\includegraphics[trim={1cm 2cm 0 2cm},clip, scale=0.085]{doubleheterostationary/cluster22.png} \caption{$t = 10.5 \; \mathrm{ms}$}
  \end{subfigure}
    \begin{subfigure}[b]{0.33\textwidth}
 \hspace*{-4em}\includegraphics[trim={1cm 2cm 0 2cm},clip, scale=0.085]{doubleheterostationary/cluster33.png} 
 \hspace*{-.6em}\includegraphics[trim={.4cm 0cm 0 0cm},clip, scale=0.17]{singlewave_stationary/scalep.png}\caption{$t = 14.8 \; \mathrm{ms}$}
  \end{subfigure}
  \vspace{-0.4cm}
  \caption{Snapshots at different times of $\tau^K$ colored with the corresponding local polynomial degree.}
  \label{fig:: double_wave_clusterhetero}
\end{figure}
\end{comment}
Moreover, the presence of the discontinuity in the conductivity tensor leads to an additional increase in the total NDof in the time period when the second wavefront passes through that specific portion of the domain (a zoom in this particular time window is reported in \ref{fig:dof_evolution_doubletvh}).
\input{heterowave}
This increase in NDofs lasts from $2ms$ up to $5ms$. After that, the number of elements with polynomial degree $p=5$ rises to capture both steep fronts accurately (see Figure \ref{fig:ndof_evolution_doublehetero}). Even in a heterogeneous contest, the adaptive algorithm can correctly identify the two waves in the domain, exploiting different local degree distributions.
%and in Figure \ref{fig:: double_wave_clusterhetero}, where the local error indicator for three different snapshots at the midpoint of each mesh element is represented. 
 \begin{figure}[h!]
 \centering
   \begin{subfigure}{\textwidth}
    \centering
    \hspace*{-.5em}\includegraphics[scale=0.18]{singlewave_stationary/scale_.png}
    \includegraphics[trim={0 0cm 0 0cm},clip, scale=0.18]{singlewave_stationary/scale_p.png}
    \includegraphics[trim={0 0.1cm 0 0.1cm},clip, scale=0.19]{doubleheterostationary/scale_tau.png}
    \end{subfigure}
 \begin{subfigure}{0.41\textwidth}
\centering
\includegraphics[trim={3cm 13cm 3cm 13cm},clip, scale=0.07]{doubleheterostationary/sol.14.png}
\includegraphics[trim={3cm 13cm 3cm 13cm},clip, scale=0.07]{doubleheterostationary/p.14.png} 
\includegraphics[trim={3cm 13cm 3cm 13cm},clip, scale=0.07]{doubleheterostationary/t.14.png}
\subcaption{$t = 1.5 \; \mathrm{ms}$}\label{fig:doublehetero01}  
 \end{subfigure}
 \begin{subfigure}{0.41\textwidth}
\centering
\includegraphics[trim={3cm 13cm 3cm 13cm},clip, scale=0.07]{doubleheterostationary/sol.35.png}
\includegraphics[trim={3cm 13cm 3cm 13cm},clip, scale=0.07]{doubleheterostationary/p.35.png}
\includegraphics[trim={3cm 13cm 3cm 13cm},clip, scale=0.07]{doubleheterostationary/t.35.png} 
\subcaption{$t = 3.6 \; \mathrm{ms}$}  
\label{fig:doublehetero0}
 \end{subfigure}
    \begin{subfigure}{0.41\textwidth}
\centering
\includegraphics[trim={3cm 13cm 3cm 13cm},clip, scale=0.07]{doubleheterostationary/sol.53.png}
\includegraphics[trim={3cm 13cm 3cm 13cm},clip, scale=0.07]{doubleheterostationary/p.53.png}
\includegraphics[trim={3cm 13cm 3cm 13cm},clip, scale=0.07]{doubleheterostationary/t.53.png} 
\subcaption{$t = 7.7 \; \mathrm{ms}$}  \label{fig:doublehetero0D}  
 \end{subfigure}
     \begin{subfigure}{0.41\textwidth}
\centering
\includegraphics[trim={3cm 13cm 3cm 13cm},clip, scale=0.07]{doubleheterostationary/sol.137.png}
\includegraphics[trim={3cm 13cm 3cm 13cm},clip, scale=0.07]{doubleheterostationary/p.137.png}
\includegraphics[trim={3cm 13cm 3cm 13cm},clip, scale=0.07]{doubleheterostationary/t.137.png} 
\subcaption{$t = 13 \; \mathrm{ms}$}  \label{fig:doublehetero0D}  
 \end{subfigure}
  \caption{Test case of Subsection~\ref{sec:HeteroCase}. Computed solution, local polynomial degree distribution and computed local error indicator defined as in Equation \eqref{eq::indicator} for different time snapshots.}
  \label{fig::ev_double_wavehetero}
\end{figure}
For the steepest and slowest wave, we observe a degree distribution similar to the homogeneous contest, with a high concentration of high degrees in a narrow domain stripe, which follows the evolution of the wave.
Figure \ref{fig::ev_double_wavehetero} shows the computed numerical solution, the corresponding local polynomial degree, and the computed local error indicator at different snapshots.
The different polynomial bands at for the two wavefronts are visible both in the evolution of the central panel in Figures \ref{fig:doublehetero01} and \ref{fig:doublehetero0D}.
At the beginning of the simulation, the less steep wave on the right-hand side of the domain shows a more spatially distributed polynomial distribution.
The mesh elements in correspondence with the wave are discretized with lower polynomial degrees, as is evident from Figure \ref{fig:doublehetero01}. 
At the jump in conductivity values, the wave speed and slope change, evolving similarly to the wave on the left, which is steeper. We note that at heterogeneity, the analysis of elements with a high degree becomes crucial, so that elements in the domain where the wave has already passed can be rechecked and discretized with lower degrees.

==> homogeneous.tex <==
\subsubsection{Homogeneous case} \label{sec:HomogCase}
This test case consists of a simulation in which both waves move with the same velocity $c = 0.5 \text{mm} \cdot \text{ms}^{-1}$.
\begin{figure}[h!]
\centering
\vspace{-0.3cm}
\begin{subfigure}[t]{0.45\textwidth}
\centering
\color{white}{test}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.45\textwidth}
\centering
\hspace*{0em}\includegraphics[trim={0cm 0cm 0cm 0cm},clip,scale=0.15]{singlewave_stationary/scale_.png}
\end{subfigure}
\begin{subfigure}[t]{0.45\textwidth}
\centering
\vspace*{-3ex}
\includegraphics[trim={2cm 13cm 2cm 13cm},clip, scale=0.075]{doublehomostationary/mesh.png}
\caption{\label{fig:double_mesh}} 
\end{subfigure}\hfill
\begin{subfigure}[t]{0.45\textwidth}
\centering
\vspace*{-3ex}
\includegraphics[trim={2cm 13cm 2cm 13cm},clip, scale=0.075]{doublehomostationary/initial_.png}
\caption{\label{fig:double_initial}} 
\end{subfigure}
    \caption{Test case of Subsection~\ref{sec:HomogCase}.  (\ref{fig:double_mesh}) computational domain corresponding polytopal grid with 1500 elements ($h = 0.1588$); (\ref{fig:double_initial}) initial condition for double traveling wavefront with $x_1=-3$ and $x_2=1.5$.}
    \label{fig:doublewave}
\end{figure}
The mesh is characterized by 1500 elements ($h = 0.1105$), and the initial condition is defined as in Equation \eqref{eq:initial_doublewave}. Figure \ref{fig:doublewave} depicts the polytopal mesh and the initial condition. The two waves evolve in opposite directions towards the center of the domain at the same speed. The adaptive algorithm correctly tracks the two wavefronts, with a high-order polynomial approximation degree employed in the proximity of the wavefronts.
%Figure \ref{fig:: double_wave_cluster}  shows the element-wise plot of the local error indicator $\tau_K$, at three different temporal instants, colored with respect to the corresponding local polynomial degree. 
\input{doublehomograph}
Also in this test case, we observe a significant reduction in the total number of degrees of freedom  (see, e.g., Figure \ref{fig:dof_evolution_doubletv}), which is a consequence of the $p$-adaptive scheme. Starting from $3.15e4$ NDoF, we reach around $8.6e3$ for the two waves traveling in the domain (with a 73\% reduction).
\begin{comment}
\begin{figure}[h]
\begin{subfigure}[b]{0.33\textwidth}
 \includegraphics[trim={1cm 2cm 0 7cm},clip, scale=0.05]{doublehomostationary/cluster1.png} \caption{$t = 1.5 \; \mathrm{ms}$}  
  \end{subfigure}
    \begin{subfigure}[b]{0.33\textwidth}
 \hspace*{-2.5em}\includegraphics[trim={1cm 2cm 0 6cm},clip, scale=0.05]{doublehomostationary/cluster2.png} \caption{$t = 10.5 \; \mathrm{ms}$}
  \end{subfigure}
    \begin{subfigure}[b]{0.33\textwidth}
 \hspace*{-4em}\includegraphics[trim={1cm 2cm 0 6cm},clip, scale=0.05]{doublehomostationary/cluster3.png}
 \hspace*{-.4em}\includegraphics[trim={.4cm 0cm 0 0cm},clip, scale=0.17]{singlewave_stationary/scalep.png}
 \caption{$t = 14.8 \; \mathrm{ms}$}
  \end{subfigure}
  \caption{Snapshots at different times of $\tau_K$ colored with respect to the corresponding local polynomial degree.}
  \label{fig:: double_wave_cluster}
\end{figure}
\end{comment}
%%%%%%%%%%%
 \begin{figure}[h!]
 \centering
 \begin{subfigure}[b]{0.14\textwidth}
\raisebox{55mm}{
  \begin{tabular}{@{}l@{}}
\footnotesize{Numerical solution} \\
    \footnotesize{$p_K = 5 \; \forall K$}
    \\[0.5cm]
\footnotesize{Numerical solution}  \\
\footnotesize{adaptive}\\[1.3cm]
\footnotesize{Polynomial} \\
\footnotesize{distribution}\\[1.4cm]
\footnotesize{$\|u_h - u_\text{ex}\|_{L^2(K)}$}\\[1.4cm]
\footnotesize{$\|u_h - u_\text{ex}\|_{DG(K)}$}\\[1.4cm]
\footnotesize{Indicator} \\
\footnotesize{distribution}
  \end{tabular}}
  \end{subfigure}
\begin{subfigure}{0.4\textwidth}
\centering
\hspace*{30ex}\includegraphics[scale=0.14]{singlewave_stationary/scale_.png}
\includegraphics[trim={1cm 13cm 1cm 13cm},clip, scale=0.07]{doublehomostationary/sol.70.png}
\includegraphics[trim={1cm 13cm 1cm 13cm},clip, scale=0.07]{doublehomostationary/sol.70.png}
\hspace*{35ex}\includegraphics[trim={0 0cm 0 0cm},clip, scale=0.16]{singlewave_stationary/scale_p.png}
\includegraphics[trim={1cm 13cm 1cm 13cm},clip, scale=0.07]{doublehomostationary/p.70.png}
\hspace*{30ex}\includegraphics[trim={0 0cm 0cm 0cm},clip, scale=0.16]{doublehomostationary/l2scaleerror.png}
\includegraphics[trim={1cm 13cm 1cm 13cm},clip, scale=0.07]{doublehomostationary/doubleL27.png} 
\hspace*{30ex}\includegraphics[trim={0 0cm 0 0cm},clip, scale=0.16]{doublehomostationary/DGscalenew.png}
\includegraphics[trim={1cm 13cm 1cm 13cm},clip, scale=0.07]{doublehomostationary/doubleDG7.png}
\hspace*{25ex}\includegraphics[trim={0 0.1cm 0 0.1cm},clip, scale=0.16]{doublehomostationary/scale_tau.png}
\includegraphics[trim={1cm 13cm 1cm 13cm},clip, scale=0.07]{doublehomostationary/t.70.png} 
\subcaption{$t = 7.1 \; \mathrm{ms}$}  
\end{subfigure}
\begin{subfigure}{0.4\textwidth}
\centering
\phantom{\includegraphics[scale=0.14]{singlewave_stationary/scale_.png}}
\includegraphics[trim={1cm 13cm 1cm 13cm},clip, scale=0.07]{doublehomostationary/sol162.png}
\includegraphics[trim={1cm 13cm 1cm 13cm},clip, scale=0.07]{doublehomostationary/sol162.png}
\phantom{\includegraphics[trim={0 0cm 0 0cm},clip, scale=0.16]{singlewave_stationary/scale_p.png}}
\includegraphics[trim={1cm 13cm 1cm 13cm},clip, scale=0.07]{doublehomostationary/p162.png}
\phantom{\includegraphics[trim={0 0cm 0cm 0cm},clip, scale=0.16]{doublehomostationary/l2scaleerror.png}}
\includegraphics[trim={1cm 13cm 1cm 13cm},clip, scale=0.07]{doublehomostationary/doubleL216.png}
\phantom{\includegraphics[trim={0 0cm 0 0cm},clip, scale=0.16]{doublehomostationary/DGscalenew.png}}
\includegraphics[trim={1cm 13cm 1cm 13cm},clip, scale=0.07]{doublehomostationary/doubleDG16.png}
\phantom{\includegraphics[trim={0 0.1cm 0 0.1cm},clip, scale=0.16]{doublehomostationary/scale_tau.png}}
\includegraphics[trim={1cm 13cm 1cm 13cm},clip, scale=0.07]{doublehomostationary/t162.png} 
\subcaption{$t = 16.6 \; \mathrm{ms}$}  
 \end{subfigure}
  \caption{Test case of Subsection~\ref{sec:HomogCase}. Computed error together with the plot of the local polynomial degree distribution and the evolution of the local error indicator defined in Equation \eqref{eq::indicator} at different time snapshots.}
  \label{fig::ev_double_wave}
\end{figure}
 Finally, when the two waves collide (approximately at $15.6 ms$), the quiescent state is discretized with linear polynomials and $4.5e3$ NDoF (with 86\% reduction). In addition, the cost of computing the local error indicator is decreased significantly due to the localized computations of the indicator for the relevant elements only, as shown in Figure \ref{fig:comptau_doubletv}.
In Figure \ref{fig::ev_double_wave}, we represent the evolution of the numerical solution, the evolution of the polynomial degree, and the computed local error indicator $\tau_K$ at different time steps.
We observe that the algorithm correctly identifies the two waves and that the polynomial distribution for the approximation is similar for both waves. This is consistent with what is expected because the two waves have the same slope and speed.  We also report the $L2$-norm  and  $DG$-norm errors defined in Equation \eqref{eq::DG_norm} computed with respect to the numerical solution obtained by the uniform method (with $p_\text{max}=5$). We observe that both local errors are extremely small, indicating an accuracy in the proposed adaptive algorithm. 
\begin{table}[h!]
    \centering
    \caption{Test case of Subsection~\ref{sec:HomogCase}. $L2$-norm and $DG$-norm for different final times. Here $u_h^\text{ad}$ is the numerical solution computed with the adaptive scheme, $u_h^\text{un}$ is the one computed with the uniform scheme ($p_K=5 \; \forall K$).}
    \label{tab:errorL2DG}
    \begin{tabular}{c|cc}
    \hline
        $T_\text{max}$ & $7.1ms$ &  $16.6ms$\\
        \hline
        $\|u_h^\text{ad} - u_h^\text{un}\|_{L^2(\Omega)}$ & $7.37e-5$ & $9.12e-5$\\
        $\|u_h^\text{ad} - u_h^\text{un}\|_{DG(\Omega)}$ & $1.8e-3$ & $2.04e-3$\\
        \hline
    \end{tabular}
\end{table}
 In particular, the error in norm $DG$ is high in correspondence with elements having neighbours discretized with different polynomial degrees; this is perfectly consistent with what we expect, given that in the $DG$-norm definition the penalty parameter defined in Equation \eqref{eq:eta} has to be considered. Furthermore, in Table \ref{tab:errorL2DG} we report the errors in the two norms for the test case presented.

==> test_case_dof.tex <==
\begin{figure}[h]
\centering
\begin{subfigure}[t]{0.45\textwidth}
\centering
\vspace*{-3ex}
\color{white}{test}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.45\textwidth}
\vspace*{-3ex}
\centering
\hspace*{1em}\includegraphics[trim={0 0cm 0 0cm},clip,scale=0.18]{photos_singlewave/scale_.png}
\end{subfigure}
\begin{subfigure}[t]{0.45\textwidth}
\centering
\vspace*{-1ex}
\includegraphics[trim={0 11cm 0 13cm},clip, scale=0.09]{photos_singlewave/mesh_.png}
\caption{Polytopal grid with 1500 elements ($h = 0.1170$).} \label{fig:comput_domain_square2}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.45\textwidth}
\centering
%\hspace*{1.8em}\includegraphics[scale=0.2]{photostv/scale_.png}
\vspace*{-1ex}
\includegraphics[trim={0 11cm 0 13cm},clip, scale=0.09]{photos_singlewave/initial_.png} \caption{Initial condition for the transmembrane potential $u$.} \label{fig:comput_domain_IC2}
\end{subfigure}
\caption{Computational domain corresponding polytopal grid, (\ref{fig:comput_domain_IC2}) initial condition of the transmembrane potential.}
\label{fig:tvinitial}
\end{figure}
%% p1
  %      err_u_L2: [1.0055 0.3082 0.0837 0.0356 0.0088]
  %      err_u_dG: [46.6285 24.5465 12.3288 7.8738 3.8335]
  %    err_Energy: [1.0163 0.3178 0.0924 0.0434 0.0150]
  %             h: [0.3615 0.2025 0.1220 0.0753 0.0374]

%% p2
  %      err_u_L2: [0.1565 0.0297 0.0044 0.0013 1.9852e-04]
  %      err_u_dG: [11.4497 3.5785 0.9118 0.3684 0.0881]
  %    err_Energy: [0.1606 0.0318 0.0053 0.0017 3.4308e-04]
  %             h: [0.3615 0.2025 0.1220 0.0753 0.0374]

%% p3

  %      err_u_L2: [0.0297 0.0030 2.5898e-04 4.9944e-05 3.9909e-06]
  %      err_u_dG: [2.8816 0.4801 0.0656 0.0178 0.0023]
  %    err_Energy: [0.0311 0.0034 3.3314e-04 7.5196e-05 8.0577e-06]
  %             h: [0.3615 0.2025 0.1220 0.0753 0.0374]


%% p4
 %       err_u_L2: [0.0046 2.7075e-04 1.2175e-05 1.3578e-06 4.7985e-08]
 %       err_u_dG: [0.5850 0.0592 0.0046 7.8357e-04 4.9525e-05]
 %     err_Energy: [0.0046 2.7140e-04 1.2261e-05 1.3805e-06 5.0350e-08]
 %              h: [0.3615 0.2025 0.1220 0.0753 0.0374]
